A Semantic Framework for the Security Analysis of Ethereum smart contracts

Smart contracts are programs running on cryptocurrency (e.g., Ethereum) blockchains, whose popularity stem from the possibility to perform financial transactions, such as payments and auctions, in a distributed environment without need for any trusted third party. Given their financial nature, bugs or vulnerabilities in these programs may lead to catastrophic consequences, as witnessed by recent attacks. Unfortunately, programming smart contracts is a delicate task that requires strong expertise: Ethereum smart contracts are written in Solidity, a dedicated language resembling JavaScript, and shipped over the blockchain in the EVM bytecode format. In order to rigorously verify the security of smart contracts, it is of paramount importance to formalize their semantics as well as the security properties of interest, in particular at the level of the bytecode being executed. In this paper, we present the first complete small-step semantics of EVM bytecode, which we formalize in the F* proof assistant, obtaining executable code that we successfully validate against the official Ethereum test suite. Furthermore, we formally define for the first time a number of central security properties for smart contracts, such as call integrity, atomicity, and independence from miner controlled parameters. This formalization relies on a combination of hyper- and safety properties. Along this work, we identified various mistakes and imprecisions in existing semantics and verification tools for Ethereum smart contracts, thereby demonstrating once more the importance of rigorous semantic foundations for the design of security verification techniques.

==> extended.tex <==
% Appendix 

\section{Formalization}

\input{formalization}

\section{Small step semantics}

\input{smallstep}


==> extendedheader.tex <==
% appendix header 

%\usepackage{amssymb}
%\usepackage{amsthm}
%\usepackage{ stmaryrd }
%\usepackage{xargs}


%\newtheoremstyle{acmplain}%
%  {.5\baselineskip\@plus.2\baselineskip
%    \@minus.2\baselineskip}% space above
%  {.5\baselineskip\@plus.2\baselineskip
%    \@minus.2\baselineskip}% space below
%  {\@acmplainbodyfont}% body font
%  {\@acmplainindent}% indent amount
%  {\@acmplainheadfont}% head font
%  {.}% punctuation after head
%  {.5em}% spacing after head
%  {\thmname{#1}\thmnumber{ #2}\thmnote{ {\@acmplainnotefont(#3)}}}% head spec
%\def\@acmdefinitionbodyfont{\normalfont}
%\def\@acmdefinitionindent{\parindent}
%\def\@acmdefinitionheadfont{\itshape}
%\def\@acmdefinitionnotefont{\@empty}
%
%\newtheoremstyle{acmdefinition}%
%  {.5\baselineskip\@plus.2\baselineskip
%    \@minus.2\baselineskip}% space above
%  {.5\baselineskip\@plus.2\baselineskip
%    \@minus.2\baselineskip}% space below
%  {\@acmdefinitionbodyfont}% body font
%  {\@acmdefinitionindent}% indent amount
%  {\@acmdefinitionheadfont}% head font
%  {.}% punctuation after head
%  {.5em}% spacing after head
%  {\thmname{#1}\thmnumber{ #2}\thmnote{ {\@acmdefinitionnotefont(#3)}}}% head spec


%\theoremstyle{plain}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\theoremstyle{definition}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{definition}[theorem]{Definition}
%\theoremstyle{acmplain}


==> properties.tex <==
In general, it should be distinguished whether a contract should be analysed from a developer's or a user's perspective. Developers may want to check that their contracts can be called with the expected behaviour in any execution environment (arbitrary arguments, call stack size etc.) while the queries of users might be more specific as they are in control of the arguments they provide to a call. 
The attacks presented in \ref{vulnerabilities} focus on bugs introduced by developers. Consequently we will focus on properties that are ensured regardless of the way contracts are called. 

%One should also take into consideration that contracts can be called in several ways: 
%\begin{enumerate}
%\item Dedicated call transactions execute the code of the account 
%\item Running code performs (self) calls
%\item Create transactions execute code given as an input in order to generate the code for the newly created contract 
%\end{enumerate}


In the following we give a formal notion of useful security properties that rule out the vulnerabilities described in section \ref{vulnerabilities}.
For the sake of a simpler presentation, we will not consider the transaction effects $\transeffects$ in the semantics as those do not influence the execution. 

Formally, we represent a contract as a tuple of the form $\contract{\contractaddress}{\contractcode}$ where $\contractaddress$ denotes the address of the contract and $\contractcode$ denotes the contract's code. We assume functions $\getcontractaddress{\cdot}$ and $\getcontractcode{\cdot}$ that extract the a contracts address and code respectively. 

In order to give concise security definitions, we introduce an annotation to the small step semantics that simplifies arguing about contract execution: We annotate every execution state with the contract that is currently executed. 
In the case of executing initialization code, we use $\bot$. 

\begin{align*}
\callstack &\define \callstackplain ~|~ \cons{\annotate{\excstate}{c}}{\callstackplain} ~|~  \cons{\annotate{\haltstate{\gstate}{\lgas}{\data}}{c}}{\callstackplain} \\
\callstackplain &\define \nil ~|~ \cons{\annotate{\regstate{\mstate}{\exenv}{\gstate}}{c}}{\callstackplain} 
\end{align*}
where $c \in \BB^{160} \times \arrayof{\BB} \cup \{ \bot \}$. 

Formally, we extend the small-step semantics in a straight-forward way to include the annotations. 

As we will argue about contracts being called in arbitrary setting, we additionally introduce the notion of a reasonable call stack. 
Intuitively, an annotated call stack is is reasonable, if it is reachable from an initial contract execution or an initialization code execution. 

\begin{definition}[Reasonability of call stacks]
An annotated call stack $\callstack$ is {\callstackvalid} if and only if one of the following condition holds for some transaction $\transaction$, some block header $\blockheader$, some global state $\gstate$, some transaction environments $\transenv$ and some transaction results $\transeffects$:
\begin{align*}
\inittrans{\transaction}{\blockheader}{\gstate} = \some{(\transenv, \exstate)} \land \ssteps{\transenv}{\exconf{\cons{\annotate{\exstate}{x}}{\nil}}{\emptytranseffects}}{\exconf{\callstack}{\transeffects}}
\end{align*}
where 
\begin{align*}
x = 
\begin{cases}
\bot & \access{\transaction}{\transactiontype} = \createtrans \\
\access{\transaction}{\recipient} &  \access{\transaction}{\transactiontype} = \calltrans
\end{cases}
\end{align*}
where $\recipient$ extracts the recipient of the transaction and $\transactiontype$ determines the type of the transaction that is either $\createtrans$ for create transaction or $\calltrans$ for call transactions.
%\begin{itemize}
%\item for some initial gas value $\lgas$, some execution environment $\exenv$, some contract $c$ and some global state $\gstate$ such that $c$ complies to $\gstate$, it holds that  \newline
%$\ssteps{\transenv}{\cons{\annotate{\regstate{\smstate{\lgas}{0}{\lam{x}{0}}{0}{\nil}}{\exenv}{\sigma}}{c}}{\nil}}{\callstack}$ 
%\item 
%%TODO  sender needs to exist and needs to have balance of at least the transaction value and a nonce of at least 1, sender and originator are the same
%for some initial gas value $\lgas$, some execution environment $\exenv$  and some global state $\gstate$, it holds that \newline
%$\ssteps{\transenv}{\cons{\annotate{\regstate{\smstate{\lgas}{0}{\lam{x}{0}}{0}{\nil}}{\exenv}{\sigma}}{\bot}}{\nil}}{\callstack}$ 
%%TODO no input data in this case 
%\end{itemize}

We extend this definition to reasonability for concrete global states by fixing the arbitrary $\gstate$ in the definition above to a concrete one $\concrete{\gstate}$ and say in this case that a call stack is reasonable for $\concrete{\gstate}$.
\end{definition}
%TODO Potentially it would be better to be even more general here: Define not only plain validness, but allow to specify some 'fixed' values (as e.g. the contract might be called with specific values) 

In addition, we introduce a substack relation $\subcallstack$ on annotated call stacks that simplifies reasoning about calls in an arbitrary environment: 

First we define concatenation ($++$) for plain (annotated) call stacks using a recursive definition: 
\begin{definition}[Concatenation of plain call stacks]
\begin{align*}
\concatstack{\nil}{\callstackplain} &= \callstackplain \\
\concatstack{\cons{\exstate}{\callstackplain}}{\callstackplain'} &= \cons{\exstate}{(\concatstack{\callstackplain}{\callstackplain'})}
\end{align*}
\end{definition}

Using concatenation, we define the substack relation: 
\begin{definition}[Substack]
The plain call stack $\callstackplain$ is a (strict) substack of $\callstack$ if there exists an execution state $\exstate$ and a plain call stack $\callstackplain'$ such that $\callstack = \cons{\exstate}{(\concatstack{\callstackplain'}{\callstackplain})}$. 
\end{definition}
The definition carries easily over to annotated call stacks. 

%TODO discussion on trace properties vs hyper properties. Later on discuss why the hyper property is checkable using z3 
\subsection{Absence of reentrancy}
A contract $c$ is not re-entrant if (when being called in an arbitrary way) it can call it self again (directly or indirectly) before its original execution has terminated. 

We formally define the absence of re-entrancy  as single-entrancy. 

\begin{definition}[Single-entrancy]
\label{single-entrancy}
A contract $c$ is single-entrant, if
for all execution states $\exstate$, $\exstate'$, all call stacks $\callstack$, $\callstack'$ such that $\cons{\annotate{\exstate}{c}}{\callstack}$ is {\callstackvalid}, for all transaction environments $\transenv$ and all $c' \in \BB^{160} \cup \{ \bot \}$ the following condition holds:
\begin{align*}
\ssteps{\transenv}{\cons{\annotate{\exstate}{c}}{\callstack}}{\cons{\annotate{\exstate'}{c'}}{\callstack'}}
\land \cons{\exstate}{\callstack} \subcallstack \callstack' \implies c \neq c'
\end{align*}
\end{definition}
%TODO maybe introduce that the stack should be well-formed 

\subsection{Correct exception handling}
The correct exception handling can be seen as purely syntactic property on the contracts byte code: After every call instruction, an $\ISZERO$ instruction is expected that checks for the success of the call. This approach is also taken by \cite{luu2016making} and a corresponding check is even incorporated in the Solidity online compiler. However, it should be mentioned that this criterion is by far neither sufficient nor necessary to ensure correct exception handling. 
Guaranteeing correct exception handling by a semantic condition is not easily possible without a precise specification of the developer's intentions. 
%TODO could one require something like: there is a difference in exceptional and non-exceptional cases? Different state? Change in the control flow? The local state changes also when a useless ISZERO command is done, the state is changed. Maybe one can express something like: ,Different code is executed: After a certain number of steps the execution will reach a different pc

\subsection{Calling known addresses}
To prevent calls to the unknown, it is sufficient if the user specifies the set of addresses it expects the contract under analysis to call. 
We define a corresponding property that ensures that the direct and indirect calls of a contract are restricted to addresses specified in the set. 
The corresponding property can be seen as a white-listing of trust-worthy contracts. 
Actually this property implies single-entrancy in the case that the contract itself is not included in the the set of specified addresses. A dual property that black lists untrusted contracts could be considered a generalization of the single-entrancy property discussed in \ref{single-entrancy}. 
%TODO but cannot express single-entrancy as it is not possible to write all addresses but c to the set. But one could establish a dual property that subsumes reentrancy (blacklisting addresses) 

\begin{definition}[Call restriction]
A contract $c$ restricts calls to a set $\callableaddresses$ of addresses if for all execution states $\exstate$, $\exstate'$, all call stacks $\callstack$, $\callstack'$ such that $\cons{\annotate{\exstate}{c}}{\callstack}$ is {\callstackvalid}, for all transaction environments $\transenv$ for all $c' \in \BB^{160} \cup \{ \bot \}$ the following condition holds:
\begin{align*}
\ssteps{\transenv}{\cons{\annotate{\exstate}{c}}{\callstack}}{\cons{\annotate{\exstate'}{c'}}{\callstack'}} \land \callstack \subcallstack \callstack' \implies \getcontractaddress{c'} \in \callableaddresses 
\end{align*}
\end{definition}

\subsection{Absence of gasless send}

To ensure that a contract never performs a gasless send, it is sufficient to check for the contract calling another contract such that no local gas is available in the initial state of the callee. 

\begin{definition}[Fuelled calls]
A contract $c$ performs only fuelled calls if for all execution states $\exstate$, $\exstate'$, all call stacks $\callstack$, $\callstack'$ such that $\cons{\annotate{\exstate}{c}}{\callstack}$ is {\callstackvalid}, for all transaction environments   $\transenv$ and for all contracts $c'$, the following condition holds: 
\begin{align*}
\ssteps{\transenv}{\cons{\annotate{\exstate}{c}}{\callstack}}{\callstack'} \land
\sstep{\transenv}{\callstack'}{\cons{\annotate{\exstate'}{c'}}{\callstack'}} \land  \callstack \subcallstack \callstack'  \\
\implies \access{\access{\exstate'}{\mstate}}{\lgas} > 0 
\end{align*}
%TODO what if s' is an exception state? This can never happen, do we need to argue here? 
\end{definition}

\subsection{Compliance to call stack limit}

In order to rule out that a contract can be called in a way that the call stack limit will be exceeded, we define a corresponding property for call stacks. 

\begin{definition}[Compliance to the call stack limit]
A contract $c$ is compliant to the call stack limit if for all execution states $\exstate$,  all call stacks $\callstack$, $\callstack'$ such that $\cons{\annotate{\exstate}{c}}{\callstack}$ is {\callstackvalid} and for all transaction environments $\transenv$, the following condition holds:
\begin{align*}
\ssteps{\transenv}{\cons{\annotate{\exstate}{c}}{\callstack}}{\cons{\annotate{\excstate}{\bot}}{\callstack'}} \land \callstack \subcallstack \cons{\annotate{\excstate}{\bot}}{\callstack'}  \\
\implies \size{\callstack'} < 1024 
\end{align*}
\end{definition}
This definition expresses the desired property as it makes use of the only way of the small step execution to exceed call stack limit. This case occurs when pushing the next execution state to the call stack in the semantics of the call rule would exceed the limit and therefore an exception state is pushed instead. 
In this single case the call stack reaches for one state the size of $1024$ and therefore indicates this particular situation. 

Note that this property does not take into consideration that the root of bugs related to exceeding the call stack limit is a wrong exception handling rather than the fact that the contract can be called in a way that makes this exception appear. 
It might be more useful to formulate a property (similar to the ones in the next section) that forbids Ether thefts due to a dependence of the contract on the call stack size. 
\subsection{Independence of unknown state}

As motivated by the attack shown in \ref{statedependency}, the developer might want to make sure that the effects of a contract execution are unaffected by certain components of the state that are not under the control of the user or that can be influenced by malicious miners. 
In particular, it is desirable that the outcome of the contract execution is independent of (parts of) the transaction environment as e.g. the block time stamp that can be determined by the miner. 
In order to avoid transaction order dependency, it is sufficient to require the outcome of a contract execution not to depend on the global state it is executed in. 

First we define independence of (parts of) the transaction environment. 
Intuitively, the effects a contract execution has on the flow of money should not be affected by (previously specified) components of the transaction environment. 

We assume $\transenvcomponents$ to be the set of the accessor functions of the transaction environment. 
We define the equality up to a component for transaction environments:
\begin{definition}[Equality up to components]
Two transaction environments $\transenv$, $\transenv'$ are equal upto component $\transenvcomponent \in \transenvcomponents$ (written $\transenv \equalupto{\transenvcomponent} \transenv'$) if 
\begin{align*}
\forall \transenvcomponent' \in \transenvcomponents / \{ \transenvcomponent \}. \; \transenvcomponent'(\transenv) = \transenvcomponent'(\transenv')
\end{align*}
\end{definition}

Additionally, we define equality on the global state for final execution states. 
\begin{definition}
Two final execution states $\exstate$ and $\exstate'$ are equal with respect to the global state ($\exstate \equalon{\gstate} \exstate'$) if for some global states $\gstate$, $\gstate'$, some gas values $\lgas$, $\lgas'$ and some output data $\data$, $\data
$ the following holds:
\begin{align*}
&\exstate = \haltstate{\gstate}{\lgas}{\data} 
\land \exstate' = \haltstate{\gstate'}{\lgas'}{\data'} \\
&\land \forall \contractaddress \in \BB^{160}. \, \gstate \, (\contractaddress) = \gstate' \, (\contractaddress)
\end{align*}
\end{definition}
%TODO

Intuitively, a contract is independent of parts of the transaction environment if two contracts called in the same way, with transaction environments that only differ in some specified components, halt in the same global state. 
This ensures in particular that the (specified) components do not influence the amount of Ether transferred between accounts during the contract execution. 
At this point one could also go for different or stronger indistinguishability properties rather then equality on the final global state. Alternative properties could e.g. require the control flow not to be distinguishable or (as done by \cite{luu2016making}) the Ether flow (opposed to the overall change in Ether) to be the same. However as transaction executions only interface via the global state, requiring that the overall effects on the global state can not be distinguished seems to be a reasonable indistinguishability property. 

\begin{definition}[Independence of the transaction environment]
A contract $c$ is independent of a subset $I \subseteq \transenvcomponents$ of components of the transaction environment if for all $\transenvcomponent \in I$, for all execution states $\exstate$, $\exstate', \exstate''$, all call stacks $\callstack$ such that $\cons{\annotate{\exstate}{c}}{\callstack}$ is {\callstackvalid}, for all transaction environments $\transenv$, $\transenv'$ the following condition holds:
\begin{align*}
& \transenvcomponent(\transenv) \neq \transenvcomponent(\transenv') 
\land \transenv \equalupto{\transenvcomponent} \transenv' \\ 
&\land \ssteps{\transenv}{\cons{\annotate{\exstate}{c}}{\callstack}}{\cons{\annotate{\exstate'}{c}}{\callstack}} 
\land \ssteps{\transenv'}{\cons{\annotate{\exstate}{c}}{\callstack}}{\cons{\annotate{\exstate''}{c}}{\callstack}} \\ 
& \land  \finalstate{\exstate'} 
\land \finalstate{\exstate''} 
\implies \exstate' \equalon{\gstate} \exstate''
\end{align*}
\end{definition}

%In order to formally capture the the independence of unknown state, we need to specify the components, we would like to allow independence of. 
%To this end, we define the set $\statecomponents$ containing the accessor functions of the components we want to prove independence of. 
%%TODO type of functions in C: should take stack and transenv. How to deal wiith Halting states? Just define functions with matching. Does not matter to much whether the functions are defined in an ugly way, we just want to have a beautiful property definition 
%
%\begin{definition}[Independence of state components]
%Let $I \subseteq \statecomponents$. 
%A contract $c$ is independent of the state components in $I$ if 
%\end{definition}
 
Next, we define independence of the global state. 
Intuitively, we want to express that the global state the contract is called in does not effect the outcome of the contract execution. 

\begin{definition}[Independence of global state]
A contract $c$ is independent of the global state if for all transaction environments $\transenv$, for all execution states $\exstate$, $\exstate'$, $\exstate''$, all call stacks $\callstack$, $\callstack'$ and all global states $\gstate$, $\gstate'$ such that $\cons{\annotate{\exstate}{c}}{\callstack}$ is {\callstackvalid} for $\gstate$ and $\cons{\annotate{\exstate}{c}}{\callstack'}$ is {\callstackvalid} for $\gstate'$, the following condition holds: 
\begin{align*}
& \gstate \neq \gstate'  \land \callstack \equalupto{\gstate} \callstack'  \\
&\land \ssteps{\transenv}{\cons{\annotate{\exstate}{c}}{\callstack}}{\cons{\annotate{\exstate'}{c}}{\callstack}} 
\land \ssteps{\transenv}{\cons{\annotate{\exstate}{c}}{\callstack'}}{\cons{\annotate{\exstate''}{c}}{\callstack'}} \\ 
& \land  \finalstate{\exstate'} 
\land \finalstate{\exstate''} 
\implies \exstate' \equalon{\gstate} \exstate''
\end{align*}
\end{definition}

In order to define equality of call stacks upto the global state ($\equalupto{\gstate}$) we first define equality of execution states up the the global state. 

\begin{definition}[Equality upto global state for execution states]
Two execution states $\exstate$, $\exstate'$ are equal upto global state ($\exstate \equalupto{\gstate} \exstate'$) if either
\begin{itemize}
\item $\exstate = \excstate = \exstate'$
\item for some global states $\gstate$, $\gstate'$, some gas value $\lgas$ and some output data $\data$ it holds that $\exstate = \haltstate{\gstate}{\lgas}{\data}$ and $\exstate' = \haltstate{\gstate'}{\lgas}{\data}$
\item for some global states $\gstate$, some machine state $\mstate$ and some execution environment $\exenv$ it holds that $\gstate'$, $\exstate = \regstate{\mstate}{\exenv}{\gstate}$ and $\exstate' = \regstate{\mstate}{\exenv}{\gstate'}$
\end{itemize}
\end{definition}

Using this definition, we can extend equality upto global state to (annotated) call stacks. 
\begin{definition}[Equality upto global state for call stacks]
Two annotated call stacks $\callstack$, $callstackb$ are equal up to global state ($\callstack 
\equalupto{\gstate} \callstackb$) if either
\begin{itemize}
\item $\callstack = \callstackb = \nil$
\item $\callstack = \cons{\annotate{\exstate}{c}}{\callstack'}$ and $\callstackb = \cons{\annotate{\exstate'}{c}}{\callstackb'}$ and $\exstate \equalupto{\gstate} \exstate'$ and $\callstack' \equalupto{\gstate} \callstackb'$.
\end{itemize}
\end{definition}

The requirement that the call stacks at the point of execution are equal upto the global states (that might be influenced by the initial global states of the transaction) requires that until this point the execution was not affected by the different global states. This captures our intuition as we do not want two contracts to be considered dependent because they are (due to a different global state) called in different ways.
%TODO problem: as the callstack incorporates the global state, letting the contracts be executed on the same call stack does not allow the initial global states to be different. So this definition is completely useless. 

%TODO at which level do we want to put the restrictions? Correctly, one should go for the state given into the initialization function and and the callee state. Does this still go along with the cool lemma? Check! 

%TODO discuss: at the moment using the notation including the valdiness we do not consider how the contract is created. I am not sure whether this is good or bad because we might know how it is created (but actually it should not be a difference once we introduce the cool extra lemma)  

Note that in contrast to the previous discussed properties, the independence properties presented in this subsection are not simple reachability properties, but hyper properties as they compare two different executions.  
\subsection{Simplifying security properties} 
In order to model the security properties introduced above in the setting of the abstract semantics, we provide some simple relaxations to the properties. 

Instead of arguing about contracts being called from {\callstackvalid} call stacks, we can argue about contracts being executed on an arbitrary call stack. The only influence the call stack potentially has on the execution is that its size might cause an error in the top-level execution due to an exceeding of the stack size limit. 

Formally, we capture this property in the following lemma: 

\begin{lemma}[Call stack indifference up to size]
Let $\exstate$ be an execution state, $c$ a contract, $\transenv$ a transaction environment and let $\callstack$, $\callstack'$ and $\callstackb$ be call stacks such that $\callstack \subcallstack \callstack'$ and $\size{\callstack} = \size{\callstackb}$. Then the following property holds:
\begin{align*}
\ssteps{\transenv}{\cons{\annotate{\exstate}{c}}{\callstack}}{\callstack'}
\Leftrightarrow \ssteps{\transenv}{\cons{\annotate{\exstate}{c}}{\callstackb}}{\concatstack{(\diffstack{\callstack'}{\callstack})}{\callstackb}}
\end{align*}
\label{call stack indifference}
\end{lemma}

where the difference on call stacks (denoted by $/$) is defined as follows: 
\begin{definition}[Difference on call stacks]
\begin{align*}
\diffstack{\callstack}{\callstackb} \define 
\begin{cases}
 \callstack' & \concatstack{\callstack'}{\callstackb} = \callstack    \\
\nil & \callstackb \not \subcallstack \callstack
\end{cases}
\end{align*}
\end{definition}

This lemma allows us to consider the contract execution in isolation of the concrete call stack and therefore independent of the execution history. When treating the call stack size explicitly (e.g. as part of the execution environment), it is possible to consider the execution on the empty call stack (but for arbitrary values for the call stack size). 

In addition, we can easily go for a local over-approximation of the execution states. Formally, the security properties are talking about {\callstackvalid} call stacks and therefore implicitly impose the condition that the call stack and therefore the execution states must be the outcomes of some valid transaction execution. 
As these restrictions anyway permit (almost) every execution state, it is reasonable to go for a simplification here. 

To this end, we extend the definition of {\callstackvalid} to execution states. 

\begin{definition}[Reasonability of execution states]
An annotated execution state $\annotate{\exstate}{c}$ is {\callstackvalid} if there is some annotated call stack $\callstack$ such that $\cons{\annotate{\exstate}{c}}{\callstack}$ is {\callstackvalid}.
\end{definition}

Additionally, we formulate a relaxation on reasonable execution states that we call well-formation.

\begin{definition}[Well-formation of annotated execution states]
An annotated execution state $\annotate{\exstate}{c}$ is well-formed if one of the following holds: 
\begin{itemize}
\item $\exstate = \excstate$
\item $\exstate = \haltstate{\gstate}{\lgas}{\data}$ and $\access{\gstate \, (\getcontractaddress{c})}{\accountcode} = \getcontractcode{c}$
\item $\exstate= \regstate{\mstate}{\exenv}{\gstate}$, $\access{\gstate \, (\getcontractaddress{c})}{\accountcode} = \getcontractcode{c}$ and \\ $\access{\exenv}{\activecode} = \getcontractcode{c}$
\end{itemize}
\end{definition} 

\begin{lemma}[Well-formation of reasonable execution states]
If an annotated execution state $\annotate{\exstate}{c}$ is {\callstackvalid}, then it is also well-formed. 
\label{well-formation of reasonable execution states}
\end{lemma}

In total, Lemma \ref{call stack indifference} and Lemma \ref{well-formation of reasonable execution states}  allow us to reason about arbitrary {\callstackvalid} execution states executing the code of the contract to be analysed being executed on the empty call stack (given an explicit modelling of the call stack size) instead of arguing about all possible ways the contracts potentially got called. 
If some state is reachable during calling contract $c$ from a reasonable call stack, then this state is reachable as well for some well-formed execution state when executing it on a arbitrary call stack of the correct size. 
Consequently when checking for non-reachability (as will be done later in the static analysis) it is sufficient to check for this property in the relaxed setting. 
%\begin{theorem}
%Let $\exstate$ be an execution state, $c$ be a contract and $\callstack$ be an annotated call stack such that $\cons{\annotate{\exstate}{c}}{\callstack}$ is a reasonable call stack. Let $\callstack'$ be an annotated call stack such that $\callstack \subcallstack \callstack'$. 
%If $\ssteps{\transenv}{\cons{\annotate{\exstate}{c}}{\callstack}}{\callstack'}$ then there is some execution state $\exstate'$ such that $\annotate{\exstate'}{c}$ is well-formed
%TODO gets quite trivial 
%\end{theorem}

%TODO this section can be probably shortened a lot by just giving a lemma/theorem that combines the lemmas in the desured way

%TODO in order to be correct we would actually also would need to require that the transaction environment and the transaction effects are 'reasonable' instead of arbitrary 

==> soundness.tex <==
%soundness proof 

For proving soundness of our analysis, we define a representation function that maps configurations into a set of horn clauses. Eventually, we will show that all steps that can be performed in the small-step semantics can be mimicked by derivations of horn clauses from the set created by the representation function. 

\subsection{Instrumented semantics}

First, we  enrich the original small step semantics with some additional information needed for the horn clause generation. 
\begin{itemize}
\item Each execution state needs to be annotated with its current global gas value. The global gas value of the bottom element on the call stack is its local gas. 
\item In the current formalization of the small step semantics, once code is loaded to the execution environment it cannot be safely tracked which account the code is originating from. So we are annotating the execution states with the it's origin contract. A contract is defined by its address and its code. 
In the cases where the code that is executed does not originate from a contract, but is a dynamically specified initialization code, we annotate the corresponding execution state with $\bot$
\item 
During contract execution new accounts might be created. We annotate execution states with the set of newly created contracts. 
\end{itemize}

Let $\contracts = \addresses \times \arrayof{\BB^8}$ denote the set of contracts. 

We obtain the following syntax for annotated call stacks: 
\begin{align*}
\callstackannotated &\define \callstackplainannotated ~|~ \cons{\annotatep{\excstate}{\ggas}{c}{\newcontracts}}{\callstackplainannotated} ~|~  \cons{\annotatep{\haltstate{\gstate}{\transeffects}{\lgas}{\data}}{\ggas}{c}{\newcontracts}}{\callstackplainannotated} \\
\callstackplainannotated &\define \nil ~|~ \cons{\annotatep{\regstate{\mstate}{\exenv}{\gstate}{\transeffects}}{\ggas}{c}{\newcontracts}}{\callstackplainannotated}
\end{align*}
where $\ggas \in \NN$, $c \in \contracts$ and $\newcontracts \subseteq \contracts$. 

\subsection{Assumptions}

\subsubsection{Codes}

We assume all codes that are potentially called to be determined by a pre-analysis. 
In general, we make a distinction between contracts that are either already present in the global state or that might get created during execution and the initialization codes that will get called in order to create new accounts. We will refer to these types of codes as contract codes and creation codes respectively. 
Instead of directly mapping contract codes to the addresses they will be referred by during the execution, we introduce internal IDs to identify contract codes as well as initialization codes. 
In the following we will denote the set of contract codes as $\callcodes$ and the set of initialization codes as $\initcodes$. 
We assume these sets to contain each code and ID only once, so they describe a partial mappings from IDs to code as well as from code to IDs. For the sake of better readability, we will denote these mappings in the following by $\getinitcodeforid{\cdot}$, $\getcallcodeforid{\cdot}$ and $\getidforinitcode{\cdot}$ and $\getidforcallcode{\cdot}$.
The connection between the IDs and the actual addresses is established by a relation $\getcallablecode{\cdot}{\cdot}$ that maps addresses to IDs. 
In addition, we assume a relation $\getinitcode{\cdot}{\cdot}{\cdot}$ that for a code ID $\id$ and a program counter value $\lpc$ gives the ID of the initialization code that will get created if the instruction at this program counter is $\CREATE$. In a similar fashion, we assume a relation $\getresultcode{\cdot}{\cdot}$ that for an initialization code ID gives the ID of the code that will get created (written to memory) when executing this code. 

We use relations instead of functions to allow program positions as well as initialization codes to create potentially different codes. 

We will later on require the following consistency property on $\callcodes$ and $\initcodes$: 
\begin{definition}[Consistency of code sets]
We call a pair of code sets $(\callcodes, \initcodes)$ consistent with respect to relations $\getcallablecode{\cdot}{\cdot}$, $\getinitcode{\cdot}{\cdot}{\cdot}$ and $\getresultcode{\cdot}{\cdot}$ if the following conditions hold: 
\begin{enumerate}
\item $\forall \id_c. \, \forall \addr. \, \getcallablecode{\addr}{\id_c} \to \exists \code. \, (\id_c, \code) \in \callcodes$
\item $\forall (\id_c, \code_c) \in \callcodes \cup \initcodes. \, \forall \id_i. \, \forall \lpc. \, \getinitcode{\id_c}{\lpc}{\id_i} \to \exists \code_i, \, (\id_i, \code_i) \in \initcodes$ 
\item $\forall (\id_i, \code_i) \in \initcodes. \, \forall \id_c. \, \getresultcode{\id_i}{\id_c} \to \exists \code_c, \, (\id_c, \code_c) \in \callcodes$
\end{enumerate}
\end{definition}

In addition, we will require $\callcodes$ and $\initcodes$ to be functional. %TODO as well injective? 

For the proof, we will restrict the execution to those executing only codes in $\callcodes$ and $\initcodes$. 
This mean that we will assume the correctness of the pre-analysis. 

\subsubsection{Hash functions}

When executing EVM byte code, for several instructions it is required to calculate the result of hash functions. 
\begin{itemize}
\item The $\SHA$ instruction offers native support for computing the Keckak-$256$ hash of a value specified on the stack. We assume the Keckak-$256$ hash function to be given by $\kec{\cdot}$. 
\item The $\BLOCKHASH$ instruction gets the hash of one of the 256 most recent complete blocks.
The block hash can be computed from the block header $\blockheader$ and the specified block number. We assume a corresponding function $\getblockhash{\cdot}{\cdot}$. 
\item The $\CREATE$ instruction requires to compute a fresh address which consists of the rightmost 160 bits of the Keckak-$256$ hash of the RLP encoding of the the address of the active account and the active account's nonce.
The corresponding function is given by $\getfreshaddress{\cdot}{\cdot}$.
\end{itemize}

As the implementation of hash functions for an SMT-solver is very bothersome and inefficient, we assume an approximation of these functions by relations. This allows for a later instantiation of the relations with arbitrary precise approximations. 

%TODO define approximations 

\begin{definition}[Approximation]
A relation $R: A \times B$ approximates a function $f: A \to B$ if the following condition holds: 
\begin{align*}
\forall a \in A. \, f\, (a) = b \to R \, (a, b)
\end{align*}
\end{definition}

We assume relations $\kecapprox{\cdot}{\cdot}$, $\blockhashapprox{\cdot}{\cdot}{\cdot}$ and $\freshaddressapprox{\cdot}{\cdot}{\cdot}$ that we will require to approximate the functions $\kec{\cdot}$, $\getblockhash{\cdot}{\cdot}$ and $\getfreshaddress{\cdot}{\cdot}$. 

\subsubsection{Jump destinations}

In addition to the pre-analysis that determines the codes that potentially get executed, we require an additional analysis that determines the set of valid jump destinations for each $\JUMP$ and $\JUMPI$ instruction. We assume a function $\jumpdests{\cdot}{\cdot}: \NN \times \NN \to \setof{\NN}$ that maps a program counter and a contract ID (specifying a point in a contract) to a set of potential jump destination (in the same contract). Similar to the pre-analysis of contract codes, we will restrict executions to those that only perform jumps according to the $\jumpdests{\cdot}{\cdot}$ function and therefore assume the correctness of the underlying pre-analysis. 

\subsection{Representation function}

We define functions that translate the call stack and the contracts that potentially get called to horn clauses. 
We split the translation into three parts: 
\begin{enumerate}
\item The translation of the codes in $\callcodes$ and $\initcodes$.
\item The translation of initial infrastructure, including the transaction environment, the approximated hash functions and the initial mapping of addresses to to internal IDs. %TODO : do we need an assumption that at least this initial mapping corresponds to the global state? 
\item The translation of call stacks. 
\end{enumerate}

\subsubsection{Translating codes}

For translating codes, in addition to the codes that should get translated, one needs the information on the potential jump destinations $\jumpdestsrel$, on the initialization codes $\initcoderel$ and on the result codes of the initialization codes $\resultcoderel$ as these are needed for the correct translation of the $\JUMP$, $\JUMPI$ and the $\CREATE$ commands. 

\begin{align*}
&\tohorncodes{\callcodes}{\initcodes}{\jumpdestsrel}{\initcoderel}{\resultcoderel} \define\\
&\{ \tohorn{\inst}{\callcodes}{\initcodes}{\jumpdestsrel}{\initcoderel}{\resultcoderel}{\id}{\lpc} ~|~ \exists \code. \,  (\id, \code) \in \callcodes \cup  \initcodes  \land \inst = \arraypos{\code}{\pc} \} \\
& \{ \pcode{\id}{\lpc}{\inst} ~|~  (\id, \code) \in \callcodes \land \arraypos{\code}{\lpc} = \inst \}
\end{align*}
%TODO with this kind of code predicate, extcode copy does not work => id (or address) needs to be parametrized. (or for all possible codes that can get called one can hardcode the rule) How can we restrict executions to those who only call  EXTCODECOPY with valid arguments? 2 approaches: either one checks for the concrete states (preconditions satisfied and so on) and excludes the wrong ones or one records the sequence of accessed codes and restrict executions to those who only access the correct codes. => Generalization of current annotations: codes touched vs codes created. 

\subsubsection{Translating the initial infrastructure}
The initial infrastructure contains information that stay unchanged during execution. This information gets translated to predicates as they are represented as non-necessarily functional relations that need to be accessed during execution. 
\begin{align*}
&\repinit{\transenv}{\kecapproxrel}{\blockhashapproxrel}{\freshaddressapproxrel} \define \\ 
&\{\ptransenv{\access{\transenv}{\originator}}{\access{\transenv}{\gasprize}}{\access{\access{\transenv}{\blockheader}}{\beneficiary}}{\access{\access{\transenv}{\blockheader}}{\difficulty}}{\access{\access{\transenv}{\blockheader}}{\blocknumber}}{\access{\access{\transenv}{\blockheader}}{\gaslimit}}{\access{\access{\transenv}{\blockheader}}{\timestamp}} \} \\
&\cup \{\pkec{v}{h} ~|~ v \in \N{256} \land h \in \N{256} \land \kecapprox{v}{h}\} \\ 
&\cup \{\pblockhash{n}{h} ~|~ n \in \N{256} \land h \in \NN \land \blockhashapprox{\access{\transenv}{\blockheader}}{n}{h} \} \\ 
&\cup \{\pfreshaddress{a}{n}{\freshaddress} ~|~ a \in \N{160} \land n \in \N{160} \land \freshaddress \in \N{160} \land  \freshaddressapprox{a}{n}{\freshaddress}  \} 
\end{align*}
%TODO change the relations to the functions. Then in the end one just needs to argue that when checking for appoximations, the values of the hash functions are correctly overapproximated 
%TODO what I am not happy about in the moment: we are creating a lot of infinite sets (this is not what is done in the implementation) 
Note that we realize the transaction environment with a predicate even though in principle accesses to it could also be hard coded in the horn clauses for the code. We do not go for this option here as in practice, queries will not be made for concrete values of the transaction environment but only loose restrictions will be put on it. This can only be expressed by formulating logical restrictions on the values of the predicate in the premise of a horn clause. The other approach is only possible if the possible values of the predicate can be enumerated. The same holds for the implementation of the hash functions. 
%TODO we should have account exists predicates per ID? Or should the id be an argument? Either we have a lot of propagation rules (for each id in C_call)? 
%Maybe one has 2 predicates: one fix callableCode_c(address) that can only get 'extended' which means that callableCode_c can get inhabited and a secound accountExists prediacte that for each address checks whether it exists (which needs to be 'call-sensitive'). One predicate is potentially more easy 
%TODO are assumptions needed that callable codes and the created states are compliant with sigma? actually we don't want require them to be completely compliant with sigma, but only when called. (one direction: for all the addresses recorded in callable codes + the newly created ones the information recorded must be the same) How is calling of addresses not determined recorded? --> requirement that only these states are allowed to be called that whose ,account annotation; is compliant with callable codes and the dynamic annotation. 
%TODO can we maybe get rid of callable code relation and somewhat shift it to the annotation (one could require in the well-formedness that the annotation always needs to include callcodes) 
%TODO Question: What is the formal justification to go for an overapproximation of the transaction environment or the global state? are we now missing the notion of abstract values? Because actually our results does not allow us to conclude that the analysis ist sound in the cases that not the precise state information was translated (but an over-approximation of it) Actually we want to argue that at least the translated predicates need to be included. I don't see how abstract values could help us. Actually, in the end, we want to argue about abstractions of the components?  Of course we can always say that by ensuring that by ensuring that 
%TODO why should we make a diffeerence between translating transenv and e.g. initcodes? exist accounts e.g gets dynamically accessed what makes it necessary to have it as a relation. About initcodes we already have assumptions (as it is a relation it can overapproximate), but transenv should be amendable to (heavy) overapproximation (e.g allowing all possible values). When they write in the android paper that they give an abstract value as argument to a predicate is this then really a symbolic value on that abstraction level or does it just mean that actually this horn clause will be translated so that for all concrete values of this abstract domain a rule will be created? If the second case hold, we would actually also like to go for abstract values. 
% Question: Do we need to be completely precise in the distinction between (condition => pred) and (for all satisfying condition: pred) Actually for stuff like transenv and the hash functions, we just want to have that there are horn clauses such that the required fact is derivable. Probably it is better to go for the concrete values in the translation (also for the horn clauses) and the argue that the soundness result still holds if the configuration is applied by something broader 
\subsubsection{Translating call stacks}
For translating call stacks, the IDs of the codes that get executed need to get extracted. This is possible as $\callcodes$ and $\initcodes$ are assumed to be injective. 
We define the following function that extracts from two sets $\callcodes$ and $\initcodes$ and a contract $c$:
\begin{align*}
\getID{c}{\callcodes}{\initcodes} 
\define \textit{let} \, c = (a, \code) \, \textit{in} \, \cond{(a = \none)}{\getidforinitcode{\code}}{\getidforcallcode{\code}}
\end{align*}
%TODO actually it would be cleaner to access the set of ids and later on argue that it is unique 

The call stack gets translated by translating the states on the stacks. As the abstract semantics does not have an explicit notion of a call stack, the different elements need  to be linked by the remaining global gas at the point of calling and the size of the stack needs to be made explicit. In addition the code annotations need to be mapped to the internal IDs. This is done by the function $\getID{\cdot}{\cdot}{\cdot}$. 
Note that for better readability, we use here a simpler stack definition that does not enforce halting and execution states to only occur as top elements. 
\begin{align*}
\repcallstack{\cons{\annotatep{\staten}{\ggas}{c}{\newcontracts}}{\cons{\annotatep{\staten}{\ggas'}{c'}{\newcontracts'}}{\callstack}}}{\callcodes}{\initcodes} &\define  
\repexstate{s}{\getID{c}{\callcodes}{\initcodes}}{g}{g'}{\size{\callstack} + 1}{\composerel{\callcodes}{\invrel{\newcontracts}}} \\
& \cup \repcallstack{\cons{\annotatep{\staten}{\ggas'}{c'}{\newcontracts'}}{\callstack}}{\callcodes}{\initcodes} \\
%&\cup \repexistingaccounts{\getID{c}{\callcodes}{\initcodes}}{}{\ggas}{\newcontracts}{\callcodes}{\initcodes} \\
\repcallstack{\cons{\annotatep{\staten}{\ggas}{c}{\newcontracts}}{\nil}}{\callcodes}{\initcodes} &\define 
\repexstate{\staten}{\getID{c}{\callcodes}{\initcodes}}{g}{\bot}{1}{\composerel{\callcodes}{\invrel{\newcontracts}}} \\
 \repcallstack{\nil}{\callcodes}{\initcodes} &\define \emptyset
\end{align*}
%\begin{align*}
%&\repcallstack{\cons{\annotatep{\excstate}{\ggas}{c}{\newcontracts}}{\cons{\annotatep{\regstaten}{\ggas'}{c'}{\newcontracts'}}{\callstackplainannotated}}}{\callcodes}{\initcodes} \define  \\
%& \qquad\{\pexception{\id}{\ggas}{\ggas'} ~|~ \id = \getID{c}{\callcodes}{\initcodes} \} \\ 
%& \qquad \cup \repcallstackplain{\cons{\annotatep{\regstaten}{\ggas'}{c'}{\newcontracts'}}{\callstackplainannotated}}{\callcodes}{\initcodes} \\
%&\repcallstack{\cons{\annotatep{\haltstate{\gstate}{\transeffects}{\lgas}{\data}}{\ggas}{c}{\newcontracts}}{\cons{\annotatep{\regstaten}{\ggas'}{c'}{\newcontracts'}}{\callstackplainannotated}}}{\callcodes}{\initcodes} \define \\ 
%&\qquad \{ \pres{\id}{g}{g'}{\pos}{v} ~|~ \id = \getID{c}{\callcodes}{\initcodes} \land \pos \in [0, \size{data} - 1] \land \arraypos{\data}{\pos} = v \}\\
%&\qquad \cup \{\preturn{\id}{g}{g'}{\size{\data}} \} \\
%& \qquad \cup \{\presgstate{\id}{g}{g'}{a}{n}{b} ~|~ \getaccount{\gstate}{a} = \account{n}{b}{\stor}{\code} \} \\
%& \qquad \cup \{\presstor{\id}{g}{g'}{a}{\pos}{v} ~|~ \getaccount{\gstate}{a} = \account{n}{b}{\stor}{\code} \land \arraypos{\stor}{\pos} = v \} \\
%& \qquad \cup \repcallstackplain{\cons{\annotatep{\regstaten}{\ggas'}{c'}{\newcontracts'}}{\callstackplainannotated}}{\callcodes}{\initcodes} \\
%&\repcallstack{\callstackplainannotated}{\callcodes}{\initcodes} \define \\ 
%&\repcallstackplain{\nil}{\callcodes}{\initcodes} \define \\
%&\repcallstackplain{\cons{\annotatep{\regstate{\mstate}{\exenv}{\gstate}{\transeffects}}{\ggas}{c}{\newcontracts}}{\callstackplainannotated}}{\callcodes}{\initcodes} \define
%\end{align*}
%TODO It is quite ugly to have two kind of stacks (rather force it inside wellformation?) => would allow to get rid of quite some cases 

%The collected contracts from the annotation get connected to the IDs of accounts that are represented
%
%\begin{align*}
%\repexistingaccounts{\id}{\ggas}{\newcontracts}{\callcodes}{\initcodes}{\lpc} &\define \{ \paccountexists{(\id, \lpc)}{g}{a}{\some{\id_a}} ~|~ (a, \code) \in \newcontracts \land \id_a = \getID{(a, \code)}{\callcodes}{\initcodes} \} \\
%& \cup \{ \paccountexists{(\id, \lpc)}{g}{a}{\none} ~|~ \forall  \code. \, (a, \code) \not \in \newcontracts \}
%\end{align*}
%TODO care about the possibility of address \none: actually we would not need the init codes here, but only call codes 

For translating the states, the different kinds of states need to be considered: 
\begin{align*}
\repexstate{\excstate}{\id}{\ggas}{\ggas_c}{n}{C} & \define \{\pexception{\id}{\ggas}{\ggas_c} \} \\
\\
\repexstate{\haltstate{\gstate}{\transeffects}{\lgas}{\dataarray}}{\id}{\ggas}{\ggas_c}{n}{C} &\define \{ \pres{\id}{g}{g'}{\pos}{v} ~|~ \pos \in [0, \size{\dataarray} - 1] \land \arraypos{\dataarray}{\pos} = v \}\\
&  \cup \{\preturn{\id}{g}{g'}{\size{\data}} \} \\
& \cup \{\presgstate{\id}{g}{g'}{a}{n}{b} ~|~ \getaccount{\gstate}{a} = \account{n}{b}{\stor}{\code} \} \\
&\cup \{\presstor{\id}{g}{g'}{a}{\pos}{v} ~|~ \getaccount{\gstate}{a} = \account{n}{b}{\stor}{\code} \land \arraypos{\stor}{\pos} = v \} \\
&\cup \{\presaccount{\id}{g}{g'}{a}{\some{\id_a}} ~|~  (a, \id_a) \in C \} \\
&\cup \{\presaccount{\id}{g}{g'}{a}{\none} ~|~  a \in \addresses \land \id_a \in \NN \land (a, \id_a) \not \in C \} \\
\\
\repstate{\regstate{\mstate}{\exenv}{\gstate}{\transeffects}}{\id}{\ggas}{\ggas_c}{n}{C} &\define 
\repgstate{\id}{\ggas}{\gstate}{\access{\mstate}{\pc}}{C}
\cup \repexenv{\id}{\ggas_c}{\exenv}{n} 
\cup \repmstate{\id}{\ggas}{\ggas_c}{\mstate} \\
\\
\repgstate{\id}{\ggas}{\gstate}{\lpc}{C} &\define \{\pgstate{(\id, \lpc)}{\ggas}{a}{n}{b} ~|~  \getaccount{\gstate}{a} = \account{n}{b}{\stor}{\code} \} \\
& \cup \{\pstor{(\id, \lpc)}{\ggas}{a}{\pos}{v} ~|~ \getaccount{\gstate}{a} = \account{n}{b}{\stor}{\code} \land \arraypos{\stor}{\pos}  =v \} \\
&\cup \{\paccountexists{(\id, \lpc)}{\ggas}{a}{\some{\id_a}} ~|~  (a, \id_a) \in C \} \\
&\cup \{\paccountexists{(\id, \lpc)}{\ggas}{a}{\none} ~|~  a \in \addresses \land \id_a \in \NN \land (a, \id_a) \not \in C \} \\
\\
\repexenv{\id}{\ggas_c}{\exenv}{n} & \define \{ \pexenv{\id}{\ggas_c}{\access{\exenv}{\activeaccount}}{\access{\exenv}{\sender}}{n}{\access{\exenv}{\tvalue}}{\size{\access{\exenv}{\inputdata}}} \} \\
&\cup \{\pindata{\id}{\ggas_c}{\pos}{v} ~|~ \arraypos{\access{\exenv}{}\inputdata}{\pos} = v \} \\
\\
\repmstate{\id}{\ggas}{\ggas_c}{\mstate} & \define  \{ \pmstate{(\id, $\access{\mstate}{\pc}$)}{\ggas}{\ggas_c}{\access{\mstate}{\gas}}{\arrayrep{\access{\mstate}{\stack}}}{\access{\mstate}{\actw}}\} \\
&\cup \{\pmem{(\id, $\access{\mstate}{\pc}$)}{\ggas}{\pos}{v} ~|~  \arraypos{\access{\mstate}{\memo}}{\pos} = v \}
\end{align*}

For translating the machine state we use the following auxiliary function translating stacks in a function representation. 
\begin{align*}
\arrayrep{\nil} &\define (0, \lam{x}{0}) \\
\arrayrep{\cons{x}{s}} & \define  \textsf{let} \, (\siz, \stackarray) = \arrayrep{s} \, \textsf{in}\, (\siz + 1, \store{\stackarray}{\siz}{x}) 
\end{align*}

\subsection{Proof}

\subsubsection{Assumptions}
For proving soundness, we need to fix several assumptions on valid execution states.
Our final goal is to restrict runs to those that only 
\begin{itemize}
\item call known contracts 
\item create known contracts
\item execute known initialization code 
\end{itemize}


\begin{definition}[Well-fomation of annotated execution states]
An annotated execution state $\annotatep{\staten}{\ggas}{(a, \code)}{\newcontracts}$ is well-formed with respect to the sets $\callcodes$ and $\initcodes$ and the relation $\getcallablecode{\cdot}{\cdot}$ if the following conditions hold: 
\begin{enumerate}
\item For all $a'$, $\id'$ it holds that if $\getcallablecode{a'}{\id'}$ holds then there is $\code'$ s.t. $(a', \code') \in \newcontracts$ and $(\id', \code') \in \callcodes$ % C_up contains the stuff specified in relation
\item If $\staten = \regstate{\mstate}{\exenv}{\gstate}{\transeffects}$ then $\code = \access{\exenv}{\activecode}$ 
\item If $a = \bot$ then it exists $\id$ s.t. $(\id, \code) \in \initcodes$
\item If $a \neq  \bot$ then exists $\id$ s.t. $(\id, \code) \in \callcodes$ % ensures that the contrat called was already created
\item $\{\code' ~|~ (a', \code') \in \newcontracts \} \subseteq \{\code' ~|~ (\id', \code') \in \callcodes \}$
\end{enumerate}
\end{definition}
%TODO why do we need to require that the code called should be in C_up? C_up at the current execution point could be much bigger than at the point of calling. It should rather be in the C_up of the callee, right? Why do we need it at alls? Case: ss calls someone that was not created before, then this execution fails (exception case of call rule applies) the same only happens in as as well when the account does not exist before => requires that C_up is compliant with sigma OR that the next step results in a non-well-formed state (as someone was called that was not even existing at this point) 
% What is about the init codes? Assume that in a CREATE an init code is written to memory and then executed. Somehow we need to ensure that the contract called there contains the init code written to the memory. By now we just enforced that the ss can only go to valid init codes. But actually we need something like: the calling state's pc and contract id needs to map to the top level code 
% what is about the result codes? Are they fully catched by the closedness property? I don't think so. We need to somehow make sure that the execution of the init code just adds contracts to C_up that comply to the one of the init code id. How can we ensure this? Could we enforce that in the halting state the resulting data (d) should be the code of some init code (yes, easy) but what about the account that got created? (link of address + code). We could annotate the execution state in additon (for the init codes) with the addresses of the account that they create. Then one could check whether the code in the halting state correctly links everything!   
% what's about jump destinations? when ss jumps to invalid jump dest, then the abstract execution just gets stuck --> no soundness! is there another way to exclude this state rather than requiring that in the case of JUMP/JUMPI, if the pre-conds for jumping are satisfied then the jumpdestination should be in the predictated set (but if we do it like this, we actually could also do it for calling and so on) Is there another way? We could assume the property of the algorithm (rather than restricting the execution) But why shouldn't we do this for the other analysis then? And would this property then be equally ugly? one could annotate the states with the pc of the previously executed command (to check for the validness of the jump, but this also comes with some overhead)
% what's about restrictions of codecopy commands
%What are we currently doing on the highlevel? Actually we want to restrict the executions only to specific runs. But in order to enforce this, we try to characterize the valid execution states that are allowed to be entered rather then directly the valid executions. Maybe we sould instead characterize the valid executions? (inserting checks on the annotations/ the auxiliary information, Cs, relations) to the rules and forbid this? I really don't know what's the most elegant way... Need to discuss! 

%Assumptions needed: 
% 1) For annotation c = (address, code), 
%  a) code is the code in I 
%  b) if address = bot then exists id s.t (id, code) \in C_init
%  c) if address != bot then exists id, s.t. (id, code) \in C_call and (address, id) \in C_up 

% code in C_call must be unique! 


%Question: how to ensure that the initcodes are compliant? Idea: If the ss makes a step to an init code (CREATE case). Then by 1 B) exists (id, code) \in C_init. and the code is the same as in I 

==> vulnerabilities.tex <==
Smart contracts are subject to several vulnerabilities that are either accidentally introduced by honest developers or integrated on purpose by  malicious contract owners. 
In the following, we give an overview of common vulnerabilities found in Ethereum smart contracts. 
Atzei at al. \cite{survey} provide a comprehensive overview of bugs in smart contracts and the levels where those bugs are introduced. Here, however we are making a different distinction with focus on the semantic security properties that are violated by the vulnerable contracts. 

%TODO bugs to introduce here: 

%
%\subsubsection{Dependency on miner controlled parameters} 
%\label{statedependency}
%Another particularity of the distributed blockchain environment is that users while performing transactions cannot make assumptions on large parts of the context their transaction will be executed in. 
%A part of this is due to the asynchronous nature of the system: it can always be that another transaction that alters the context was performed first. But actually, the situation is even more delicate as transactions are not processed in a first-come-first-serve manner, but miners have a big influence on the execution context of transactions. They can decide upon the order of the transactions in a block (and also sneak their own transactions in first) and in addition they can even control some parameters as the block timestamp within a certain range. 
%%TODO are there more? 
%Consequently, contracts whose (outgoing) money flows depend either on miner controlled block information or on state information (as the state of their storage or their balance) that might be changed by other transactions are prone to manipulations by miners. A typical example adduced in the literature is the use of block time stamps as source of randomness \cite{survey, oyente}. In a classical lottery implementation that randomly pays out to one of the participants and uses the block time\REMOVEMfor{CY}{171125}{ }stamp as source of randomness, a malicious miner can easily influence the result in his favor by selecting a beneficial timestamp. 
%
%\subsubsection{Calls to untrusted addresses}
%Even though the Solidity syntax conveys the impression of being able to communicate with well-defined contract instances, this is not necessarily the case. If a contract shall interact with an already existing contract on the blockchain, the developer needs to specify the address of this contract or the contract address needs to be derived dynamically from the context. Both these approaches are error-prone and may lead to money transfers or to code executions that were not intended by the user. 
%
%Consider the following example: 
%\begin{lstlisting}
%contract FriendlyMoney { 
%	address friend = 0xBa8AA02Fec8d3D440B3A1B60edDAAD80521581c9; 
%	
%	function sendMoneyToMyFriend(uint amount){ 
%		DonateMeMoney(friend).donate(amount); 
%	}
%}
%\end{lstlisting}
%Specifying that a contract is an instance of a certain class (as done by \lstinline|DonateMeMoney(friend)|) does not imply any run time checks, but only facilitates the calling of its functions. If at the specified address no contract of the of the specified form can be found, the callback function of the account at this address will be executed. Consequently, giving a wrong \lstinline|friend| address might not only result in sending money to the wrong account, but also in executing untrusted code. 
%
%These considerations highlight the tricky nature of Solidity semantics and motivate the importance of a precise semantic model for rigorous security reasoning. 

